Toward matrix multiplication for deep learning inference on the Xilinx Versal

The remarkable positive impact of Deep Neural Networks on many Artificial Intelligence (AI) tasks has led to the development of various high performance algorithms as well as specialized processors and accelerators. In this paper we address this scenario by demonstrating that the principles underlying the modern realization of the general matrix multiplication (GEMM) in conventional processor architectures, are also valid to achieve high performance for the type of operations that arise in deep learning (DL) on an exotic accelerator such as the AI Engine (AIE) tile embedded in Xilinx Versal platforms. In particular, our experimental results with a prototype implementation of the GEMM kernel, on a Xilinx Versal VCK190, delivers performance close to 86.7% of the theoretical peak that can be expected on an AIE tile, for 16-bit integer operands.

==> sections/conclusion.tex <==
\section{Final Discussion and Future Work}
\label{sec:remarks}


In this work, we have designed a prototype \gemm kernel that follows the ideas of GotoBLAS2,
matching the different data transfers of the algorithm across the memory
hierarchy of the Versal VCK190 ACAP as well as developing an appropriate micro-kernel
(to operate with \textcolor{black}{INT16} input data) on the AIE tile. 
%$  
From the practical point of view, 
we have demonstrated that,
by carefully choosing 
the ``cache'' configuration parameters,
this design achieves  about  \textcolor{black}{28} MACs per cycle, 
which corresponds to 86.7\% of the AIE peak performance 
\textit{when using the} \texttt{mac16()} \textcolor{black}{(advanced level AI Engine Intrinsic)~\cite{AIEintrinsics}}.
%  
\textcolor{black}{This low level library provides detailed control of the implementation, as well as close-to-peak performance.}
In future work, we plan to address the following aspects:
\begin{description}
\item[INT8 based Advanced intrinsics.]

    \textcolor{black}{% 
    The current INT16 delivers 32 MACs per cycle, yet lower precision datatypes such as INT8 can deliver up to 128 MACs per cycle. 
    Our initial implementation, with the $m_r \times n_r = 16 \times 4$ micro-kernel
      and INT16 operands, delivers performance close to the theoretical peak for INT16 when 
      $k_c$ sufficiently large.
      The design of an INT8-based micro-kernel and its integration into the \gemm algorithm is ongoing work.
      }


 \item[Exploiting multiple AIE tiles.]
      At this point we recognize that a high performance implementation of \gemm for
      an AIE-enabled Versal should target all AIE tiles in the system. Doing so
      for a platform with a very large count of tiles without hitting a hard memory wall due to
      the data accesses is a very challenging task yet inescapable objectives.
      For this purpose, we expect that it becomes primordial to exploit the 
      high speed interconnection among
      tiles to exchange the data in the local memories.
 
\end{description}



